A Blueprint for the Milky Way's Stellar Populations. V. 3D Local Dust Extinction

Using a grid of empirically calibrated synthetic spectra developed in our previous study, we construct an all-sky 3D extinction map from the large collection of low-resolution XP spectra in Gaia DR3. Along each line of sight, with an area ranging from $0.2$ to $13.4$ deg$^2$, we determine both the reddening and metallicity of main-sequence stars and model the foreground extinction up to approximately $3$ kpc from the Sun. Furthermore, we explore variations in the total-to-selective extinction ratio in our parameter search and identify its mean systematic change across diverse cloud environments in both hemispheres. In regions outside the densest parts of the clouds, our reddening estimates are validated through comparisons with previous reddening maps. However, a notable discrepancy arises when compared to other independent work based on XP spectra, although our metallicity scale shows reasonable agreement with the high-resolution spectroscopic abundance scale. We also assess the accuracy of the XP spectra by applying our calibrated models, and confirm an increasing trend of flux overestimation at shorter wavelengths below $400$ nm.

==> tab2_full.tex <==
\begin{deluxetable}{lll}
\tablecaption{A Family of Solutions on Stellar Parameters\label{tab:tab2}}
\tabletypesize{\scriptsize}
\tablehead{
   \colhead{Wavelength} &
   \colhead{Mean deviation} &
   \colhead{Std.\ deviation} &
   \colhead{Median frac. uncertainty} \\
   \colhead{(nm)} &
   \colhead{} &
   \colhead{} &
   \colhead{}
}
\startdata
    336 &  0.412 & 0.476 & 0.266 \\
    345 &  0.087 & 0.189 & 0.162 \\
    354 &  0.128 & 0.240 & 0.185 \\
    363 & -0.075 & 0.103 & 0.165 \\
    372 &  0.058 & 0.121 & 0.175 \\
    381 &  0.065 & 0.169 & 0.251 \\
    390 &  0.018 & 0.112 & 0.190 \\
    399 & -0.034 & 0.056 & 0.087 \\
    408 & -0.011 & 0.043 & 0.058 \\
    417 &  0.020 & 0.041 & 0.051 \\
    426 & -0.015 & 0.045 & 0.056 \\
    435 & -0.030 & 0.042 & 0.050 \\
    444 &  0.007 & 0.029 & 0.040 \\
    453 &  0.013 & 0.028 & 0.034 \\
    462 &  0.027 & 0.029 & 0.030 \\
    471 & -0.013 & 0.027 & 0.029 \\
    480 &  0.007 & 0.024 & 0.026 \\
    489 & -0.036 & 0.023 & 0.025 \\
    498 & -0.007 & 0.021 & 0.024 \\
    507 &  0.003 & 0.024 & 0.024 \\
    516 & -0.019 & 0.026 & 0.024 \\
    525 &  0.021 & 0.021 & 0.021 \\
    534 & -0.000 & 0.019 & 0.020 \\
    543 & -0.020 & 0.018 & 0.018 \\
    552 & -0.005 & 0.017 & 0.018 \\
    561 & -0.003 & 0.016 & 0.016 \\
    570 & -0.010 & 0.016 & 0.016 \\
    579 &  0.002 & 0.016 & 0.014 \\
    588 & -0.008 & 0.015 & 0.014 \\
    597 & -0.006 & 0.016 & 0.012 \\
    606 &  0.003 & 0.014 & 0.012 \\
    615 &  0.007 & 0.014 & 0.011 \\
    624 &  0.011 & 0.014 & 0.011 \\
    633 &  0.032 & 0.013 & 0.010 \\
    642 &  0.018 & 0.017 & 0.021 \\
    651 & -0.001 & 0.019 & 0.026 \\
    660 & -0.023 & 0.019 & 0.025 \\
    669 & -0.001 & 0.017 & 0.023 \\
    678 & -0.003 & 0.017 & 0.022 \\
    687 & -0.013 & 0.017 & 0.022 \\
    696 & -0.005 & 0.015 & 0.021 \\
    705 & -0.012 & 0.015 & 0.020 \\
    714 & -0.010 & 0.015 & 0.020 \\
    723 & -0.003 & 0.015 & 0.020 \\
    732 & -0.015 & 0.014 & 0.020 \\
    741 & -0.005 & 0.014 & 0.019 \\
    750 & -0.009 & 0.014 & 0.019 \\
    759 &  0.000 & 0.015 & 0.019 \\
    768 & -0.007 & 0.015 & 0.019 \\
    777 &  0.012 & 0.015 & 0.019 \\
    786 &  0.001 & 0.015 & 0.019 \\
    795 &  0.009 & 0.014 & 0.019 \\
    804 & -0.007 & 0.014 & 0.019 \\
    813 & -0.003 & 0.014 & 0.018 \\
    822 & -0.005 & 0.014 & 0.018 \\
    831 & -0.006 & 0.014 & 0.018 \\
    840 & -0.003 & 0.015 & 0.019 \\
    849 & -0.011 & 0.016 & 0.021 \\
    858 &  0.007 & 0.016 & 0.021 \\
    867 & -0.008 & 0.015 & 0.020 \\
    876 & -0.002 & 0.016 & 0.021 \\
    885 &  0.024 & 0.018 & 0.023 \\
    894 &  0.006 & 0.018 & 0.024 \\
    903 &  0.011 & 0.018 & 0.023 \\
    912 &  0.005 & 0.019 & 0.026 \\
    921 & -0.007 & 0.021 & 0.029 \\
    930 &  0.008 & 0.021 & 0.029 \\
    939 &  0.012 & 0.024 & 0.033 \\
    948 & -0.006 & 0.026 & 0.037 \\
    957 &  0.008 & 0.026 & 0.038 \\
    966 &  0.028 & 0.032 & 0.046 \\
    975 & -0.013 & 0.032 & 0.050 \\
    984 & -0.029 & 0.039 & 0.061 \\
    993 &  0.020 & 0.048 & 0.073 \\
   1002 &  0.044 & 0.058 & 0.085 \\
   1011 &  0.004 & 0.103 & 0.148 \\
\enddata
\end{deluxetable}

